MOJAVE: XV. VLBA 15 GHz Total Intensity and Polarization Maps of 437 Parsec-Scale AGN Jets From 1996-2017

We present 5321 milliarcsecond-resolution total intensity and linear polarization maps of 437 active galactic nuclei (AGNs) obtained with the VLBA at 15 GHz as part of the MOJAVE survey, and also from the NRAO data archive. The former is a long-term program to study the structure and evolution of powerful parsec-scale outflows associated with AGNs. The targeted AGNs are drawn from several flux-limited radio and gamma-ray samples, and all have correlated VLBA flux densities greater than about 50 mJy at 15 GHz. Approximately 80% of these AGNs are associated with gamma-ray sources detected by the Fermi LAT instrument. The vast majority were observed with the VLBA on 5 to 15 occasions between 1996 January 19 and 2016 December 26, at intervals ranging from a month to several years, with the most typical sampling interval being six months. A detailed analysis of the linear and circular polarization evolution of these AGN jets are presented in other papers in this series.

==> maptablestub.tex <==
%\documentclass[12pt,preprint]{aastex} 
%\newcommand{\n}{\nodata} 
%\begin{document} 
\begin{landscape} 
\begin{deluxetable}{llllcrrcccccrc} 
\tablecolumns{14} 
\tabletypesize{\scriptsize} 
\tablewidth{0pt}  
\tablecaption{\label{maptable}Summary of 15 GHz Image Parameters}  
\tablehead{ & &  & 
\colhead{$B_\mathrm{maj}$} &\colhead{$B_\mathrm{min}$} & \colhead{$B_\mathrm{pa}$} &  
\colhead{$I_\mathrm{tot}$} &  \colhead{$\sigma_\mathrm{I}$}  &  \colhead{$I_\mathrm{base}$} & 
\colhead{$P_\mathrm{tot}$} & \colhead{$\sigma_\mathrm{Q,U}$}  & \colhead{$P_\mathrm{base}$}&\colhead{EVPA} &  \colhead{Fig.} \\ 
\colhead{Source} & \colhead{Alias} & \colhead {Epoch} & 
\colhead{(mas)} &\colhead{(mas)} & \colhead{(\arcdeg)} &  
\colhead{(mJy)} & \colhead{(mJy} & \colhead{(mJy}  &  \colhead{(mJy) } &   \colhead{(mJy}  &  \colhead{(mJy }& \colhead{(\arcdeg)} & \colhead{Num.} \\ 
 &  &  &   & 
 & &   
 & \colhead{beam$^{-1}$)}  &  \colhead{beam$^{-1}$)} & & \colhead{beam$^{-1}$)}  &  \colhead{beam$^{-1}$)} & & \\ 
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} &  
\colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)} & \colhead{(9)}& \colhead{(10)} &  \colhead{(11)} & \colhead{(12)} &   \colhead{(13)} &  \colhead{(14)} } 
\startdata 
0003+380 & S4 0003+38  & 2006 Mar 9 & 1.01 & 0.73 & 18 & 650 & 0.44 & 1.15 & 16 & 0.45 & 1.48 & $78$  & 4.1   \\ 
 &   & 2006 Dec 1 & 0.85 & 0.58 & $-$17 & 512 & 0.41 & 1.10 & 9.2 & 0.46 & 1.42 & $146$  & 4.2   \\ 
 &   & 2007 Mar 28 & 0.86 & 0.61 & $-$15 & 604 & 0.33 & 0.80 & 5.6 & 0.35 & 1.08 & $144$  & 4.3   \\ 
 &   & 2007 Aug 24 & 0.92 & 0.58 & $-$28 & 555 & 0.25 & 0.80 & 7.3 & 0.30 & 0.88 & $166$  & 4.4   \\ 
 &   & 2008 May 1 & 0.82 & 0.57 & $-$9 & 808 & 0.24 & 0.70 & 12 & 0.26 & 0.84 & $178$  & 4.5   \\ 
 &   & 2008 Jul 17 & 0.84 & 0.55 & $-$12 & 727 & 0.22 & 0.60 & 17 & 0.25 & 0.79 & $175$  & 4.6   \\ 
 &   & 2009 Mar 25 & 0.84 & 0.62 & $-$12 & 435 & 0.16 & 0.50 & 10 & 0.17 & 0.56 & $145$  & 4.7   \\ 
 &   & 2010 Jul 12 & 0.89 & 0.54 & $-$12 & 438 & 0.17 & 0.50 & 10 & 0.19 & 0.63 & $132$  & 4.8   \\ 
 &   & 2011 Jun 6 & 0.91 & 0.54 & $-$10 & 605 & 0.18 & 0.50 & 2.1 & 0.20 & 0.63 & $108$  & 4.9   \\ 
 &   & 2013 Aug 12 & 0.84 & 0.53 & $-$4 & 668 & 0.20 & 0.50 & 9.8 & 0.21 & 0.75 & $139$  & 4.10   \\ 
0003$-$066 & NRAO 005  & 2003 Feb 5 & 1.32 & 0.53 & $-$6 & 2842 & 0.31 & 1.40 & 103 & 0.37 & 1.00 & $17$  & 4.11   \\ 
 &   & 2004 Jun 11 & 1.30 & 0.49 & $-$7 & 3273 & 0.32 & 1.40 & 255 & 0.61 & 1.57 & $22$  & 4.12   \\ 
 &   & 2005 Mar 23 & 1.32 & 0.53 & $-$5 & 3034 & 0.27 & 1.50 & 129 & 0.32 & 1.38 & $4$  & 4.13   \\ 
 &   & 2005 Jun 3 & 1.37 & 0.53 & $-$8 & 3017 & 0.23 & 1.40 & 110 & 0.30 & 1.00 & $175$  & 4.14   \\ 
\enddata 
\tablecomments{Columns are as follows: (1) B1950 name, (2) other name, (3) date of VLBA observation, (4) FWHM major axis of restoring beam (milliarcseconds), (5) FWHM minor axis of restoring beam (milliarcseconds), (6) position angle of major axis of restoring beam (degrees), (7) total cleaned I flux density (mJy),  (8) rms noise level of Stokes I image (mJy per beam), (9) lowest I contour level (mJy per beam), (10) total cleaned P flux density (mJy), or upper limit, based on 3 times the P rms noise level,  (11) average of blank sky rms noise level in Stokes Q and U images (mJy per beam), (12) lowest linear polarization contour level (mJy per beam), (13) integrated electric vector position angle (degrees), (14) figure number.}

\tablenotetext{a}{NRAO archive epoch}

\end{deluxetable} 
\end{landscape} 

%\end{document} 

